Walking Under the Ladder Logic: PLC-VBS, a PLC Control Logic Vulnerability Discovery Tool

Cyber security risk assessments provide a pivotal starting point towards the understanding of existing risk exposure, through which suitable mitigation strategies can be formed. Where risk is viewed as a product of threat, vulnerability, and impact, understanding each element is of equal importance. This can be a challenge in Industrial Control System (ICS) environments, where adopted technologies are typically not only bespoke, but interact directly with the physical world. To date, existing vulnerability identification has focused on traditional vulnerability categories. While this provides risk assessors with a baseline understanding, and the ability to hypothesize on potential resulting impacts, it is high level, operating at a level of abstraction that would be viewed as incomplete within a traditional information system context. The work presented in this paper takes the understanding of ICS device vulnerabilities one step further. It offers a tool, PLC-VBS, that helps identify Programmable Logic Controller (PLC) vulnerabilities, specifically within logic used to monitor, control, and automate operational processes. PLC-VBS gives risk assessors a more coherent picture about the potential impact should the identified vulnerabilities be exploited; this applies specifically to operational process elements.

==> Sections/background.tex <==
\section{PLC Program Structures}
\label{PLCbackground}
In setting out an approach by which vulnerabilities derived from current PLC programming practices can be identified, it is important first to understand the baseline construction of PLC programs.

While PLCs are available from multiple vendors, and are deployed across diverse industrial contexts (e.g., water, electricity, and gas)~\citep{Stouffer2015}, they all execute a series of instructions, referred to as a "Program". This program is, however, more commonly referred to as "control logic", and thus will be the adopted term throughout the remainder of this paper. 

Control logic acts as the intelligence behind operational process monitoring, control, and automation, enacted through its ability to interface with sensors and actuators. While this may be its primary function, the way in which it can be achieved, and the range of additional capabilities it offers, is often overlooked; for example, it can also include the configuration and operation of network protocols, hardware interfaces, SMS alerting, PLC-to-PLC data exchanges, and so on.

Using BSI/IEC standard 61131-3:2013~\citep{BritishStandardsInstitute2013} as a guide, five control logic programming languages are defined for use on PLCs (Ladder Diagrams, Function Block Diagrams, Sequential Function Charts, Instruction Lists, and Structured Text). While vendors may choose to develop their own custom languages, they are typically subtle variations of those defined by BSI/IEC. Moving one step further into the control logic ecosystem, we have Program Organization Units (POUs), applicable across all of the aforementioned languages. The following POU definitions are taken from \cite{green2021} who use and expand on BSI/IEC 61131-3. We have opted to include this extended definition as it captures one critical element not well covered by BSI/IEC 61131-3, that of variables.

\vspace{-5pt}
\begin{itemize}
	\itemsep0em
	\item \textbf{Programs}: are the highest level of organizational unit. They control the operation sequence, enabling responses to cyclic, time-based, or interrupt-driven events during program execution.  They are composed of specific instructions but also Function Blocks and Functions.
	\item \textbf{Function Blocks (FB)}: contain code that stores their values permanently in memory, remaining available post Function Block execution.
	\item \textbf{Functions}: provide discrete common functionality, for example, ADD or SQRT. Function POUs can use global variables to permanently store data, but do not have their own dedicated memory (i.e., local variables).
	\item \textbf{Variable Blocks (VB)}: store program data in the PLCs memory and can be global (gVB) or local (fVB). The latter of these are associated with Function Blocks to provide long term data storage. The VB is an addition to the POU model as defined by IEC 61131-3. This standard describes the use of variables in a general way, with limited links to their storage.
\end{itemize}
\vspace{-5pt}

Control logic can be written in three POUs: these are Programs, FBs, and Functions. Figure~\ref{fig:ladder} depicts a basic Ladder Diagram example. This control logic represents two 'if' statements. (1) If Example\_Input\_1 and Example\_Input\_2 == 1, then Set Example\_Output to 1, and (2) If Example\_Input\_1 and Example\_Input\_2 == 0, then Reset Example\_Output to 0. While this example was constructed using a Ladder Diagram, any of the five programming languages defined in BSI/IEC 61131-3 could have been adopted here (dependent on device/vendor support). Furthermore, despite any variation in language, the inputs and output variables would have remained constant. In this example, the inputs and output represent three Boolean variables stored within a gVB.

\begin{figure}[h!]
	\begin{center}
    	\includegraphics[width=1\columnwidth]{Images/exampleladder.png}
	\end{center}
    %\vspace{-2\baselineskip}
    \caption{Ladder Diagram Example}
    \label{fig:ladder}
    \vspace{-5pt}
\end{figure}

Additional specialist control logic elements for accessing and addressing system components may also exist depending on the device/vendor; these include peripherals, timers, and pointers. Pointers are perhaps the most common and well understood, due to their use within conventional programming languages. They assist in the reduction of common data replication across a control logic base (induced through other data access/processing methods).

To support the development of control logic, vendors often produce libraries of Functions and FBs~\citep{Siemens2019}; these are also referred to as "instruction sets"~\citep{AllenBradley2008}. Libraries contain pre-written control logic supporting a wide range of functions, from converter operations to communication exchanges. Due to the benefits brought about through the use of libraries (tested, trusted, standardised code snippets that provide significant time and performance efficiencies); their adoption is widespread~\citep{Ljungkrantz2007}.


